One Bug, Hundreds Behind: LLMs for Large-Scale Bug Discovery

Fixing bugs in large programs is a challenging task that demands substantial time and effort. Once a bug is found, it is reported to the project maintainers, who work with the reporter to fix it and eventually close the issue. However, across the program, there are often similar code segments, which may also contain the bug, but were missed during discovery. Finding and fixing each recurring bug instance individually is labor intensive. Even more concerning, bug reports can inadvertently widen the attack surface as they provide attackers with an exploitable pattern that may be unresolved in other parts of the program. In this paper, we explore these Recurring Pattern Bugs (RPBs) that appear repeatedly across various code segments of a program or even in different programs, stemming from a same root cause, but are unresolved. Our investigation reveals that RPBs are widespread and can significantly compromise the security of software programs. This paper introduces BugStone, a program analysis system empowered by LLVM and a Large Language Model (LLM). The key observation is that many RPBs have one patched instance, which can be leveraged to identify a consistent error pattern, such as a specific API misuse. By examining the entire program for this pattern, it is possible to identify similar sections of code that may be vulnerable. Starting with 135 unique RPBs, BugStone identified more than 22K new potential issues in the Linux kernel. Manual analysis of 400 of these findings confirmed that 246 were valid. We also created a dataset from over 1.9K security bugs reported by 23 recent top-tier conference works. We manually annotate the dataset, identify 80 recurring patterns and 850 corresponding fixes. Even with a cost-efficient model choice, BugStone achieved 92.2% precision and 79.1% pairwise accuracy on the dataset.

==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> fig/BugfindingTest.tex <==
\setlength{\fboxsep}{0.8pt}
\begin{tabular}{l|l|l|l|l|l|l}
\toprule
\textbf{Model}	&	\textbf{Memory leak} & \textbf{Incorrect NULL Check} & \textbf{Use after free} & \textbf{DF} & \textbf{SLEEP} & \textbf{PERM} \\ \hline	
granite-13b-chat-v2	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}	
&	
 \colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
 & 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}
 &	
 \colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}
 &	
 \colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B} \colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
 & 
 \colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N} \\ \hline


granite-20b-code-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}	
&	
 \colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}
& 
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{orange!20}{O}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline





granite-34b-code-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}	
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N} 
&  
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
 \colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline


codellama-34b-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}	
& 
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}	 
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{orange!20}{O}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B} \colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline





llama-2-70b-chat-q	&	\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\hspace{1.5pt}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}	
&	
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B} 
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
& 
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline



mixtral-8x7b-instruct-v01 	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}	
&	
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B} 
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{orange!20}{O}\colorbox{orange!20}{O}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline


llama-3-8b-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}	
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N} 
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
 \colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline






lama-3-70b-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}	
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\\ \hline







gpt-4o &
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\\ \hline
\bottomrule
\end{tabular}\\


==> fig/BugfindingTestIssueSummary.tex <==
\begin{tabular}{l|l|l|l|l|l|l|l|l|l}
\toprule
\textbf{Model}	&	\textbf{Hal} & \textbf{CF} & \textbf{VN} & \textbf{Hig} &	\textbf{Inc} & \textbf{FI} & \textbf{AxR} & \textbf{SE} & \textbf{NR}\\ \hline	
granite-13b-chat-v2 	&	35	& 12 & 2	& 17 & & & & &\\ \hline
granite-20b-code-instruct  	&	23	& 3	 & & 14 & 3 & 12	& 3 & 6 &\\ \hline
granite-34b-code-instruct  	&	12	& 10	 &  & & 1 &	& & 2 & 22 \\ \hline
codellama-34b-instruct	&	30	& 	10 & & 20 & 1 &	& 5 & 10 &\\ \hline
llama-2-70b-chat-q	&	43	&	8 & 	& 20 & & & & 10 & \\ \hline
mixtral-8x7b-instruct-v01 	&	6	& 10	&  & 2 & 	 & & 5 & 7 & \\ \hline
llama-3-8b-instruct	&	9	&	10 & 1	& & 1 & & 3 & 4 & \\ \hline
llama-3-70b-instruct	&	1	&8	& & & & 	&  & 5 & \\ \hline

gpt-4o 	&		& 5	&  &  & 	 & & 1 &  & \\ \hline
\bottomrule
\end{tabular}

==> fig/BugfindingTestPatch.tex <==
\setlength{\fboxsep}{0.8pt}
\begin{tabular}{l|l|l|l|l|l|l}
\toprule
\textbf{Model}	&	\textbf{Memory leak} & \textbf{Incorrect NULL Check} & \textbf{Use after free} & \textbf{DF} & \textbf{SLEEP} & \textbf{PERM} \\ \hline	
granite-13b-chat-v2	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}	
&	
 \colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
 & 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
 &	
 \colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}
 &	
 \colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B} \colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
 & 
 \colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N} \\ \hline


granite-20b-code-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}	
&	
 \colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
& 
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}
& 
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{orange!20}{O}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline





granite-34b-code-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}	
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B} 
&  
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
 \colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline


codellama-34b-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}	
& 
\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}	 
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B} \colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline





llama-2-70b-chat-q	&	\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\hspace{1.5pt}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}	
&	
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B} 
& 
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
& 
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline



mixtral-8x7b-instruct-v01 	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}	
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N} 
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{orange!20}{O}\colorbox{orange!20}{O}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline


llama-3-8b-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}	
&	
\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B} 
& 
\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
 \colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\\ \hline






lama-3-70b-instruct	&	\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}	
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}\colorbox{red!20}{N}
&	
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}
& 
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\\ \hline







gpt-4o &
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{red!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{red!20}{B}\colorbox{green!20}{N}\colorbox{red!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{red!20}{N}
&
\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{N}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\colorbox{green!20}{B}\\ \hline
\bottomrule
\end{tabular}\\


==> fig/CodePatchTokenSize.tex <==
\begin{tabular}{l|l|l|l}
\toprule
\textbf{Model}	&	\textbf{AVG Tokens} & \textbf{Medium tokens} &\textbf{(>99\%) tokens}\\ \hline	
Functions	&	164	&	74 & 1270	\\ \hline
Patch comments 	&	191	&	129 & 1400	\\ \hline
Patch code changes  	&	284	&	69 &  3100	\\ \hline
Git commits comments	&	159	& 115	 & 950	\\ \hline
Git commits code changes	&	1029	&	132 & 10000	 \\ \hline
\bottomrule
\end{tabular}

==> fig/TokenSize.tex <==
\begin{tabular}{l|l|l|l}
\toprule
\textbf{Model}	&	\textbf{Token limit} & \textbf{Max new tokens} &\textbf{Model Type}\\ \hline	
codellama-34b-instruct  	&	16384	&	4096 & Code, Decoder only	\\ \hline
granite-13b-chat-v2  	&	8192	&	4096 & Chat, Decoder only	\\ \hline
granite-20b-code-instruct  	&	8192	&	4096 &  Code	\\ \hline
granite-34b-code-instruct 	&	8192	&	4096 & Code	\\ \hline
granite-8b-code-instruct	&	4096	&	1536 &	Code \\ \hline
llama-2-70b 	&	4096	&	1536 &	Base, Decoder-only \\ \hline
llama-2-70b-chat-q   	&	4096	&	4095	& Quantized, Chat \\ \hline
llama-3-70b-instruct  	&	8192	&	2048 &	Instruct \\ \hline
llama-3-8b-instruct	&	8196	&	2048 &	Instruct \\ \hline
mixtral-8x7b-instruct-v01 &	32768	&	16384 & Decoder-only, Instruct	\\ \hline
\bottomrule
\end{tabular}
